ZerO Initialization: Initializing Neural Networks with only Zeros and Ones

Deep neural networks are usually initialized with random weights, with adequately selected initial variance to ensure stable signal propagation during training. However, selecting the appropriate variance becomes challenging especially as the number of layers grows. In this work, we replace random weight initialization with a fully deterministic initialization scheme, viz., ZerO, which initializes the weights of networks with only zeros and ones (up to a normalization factor), based on identity and Hadamard transforms. Through both theoretical and empirical studies, we demonstrate that ZerO is able to train networks without damaging their expressivity. Applying ZerO on ResNet achieves state-of-the-art performance on various datasets, including ImageNet, which suggests random weights may be unnecessary for network initialization. In addition, ZerO has many benefits, such as training ultra deep networks (without batch-normalization), exhibiting low-rank learning trajectories that result in low-rank and sparse solutions, and improving training reproducibility.

==> algorithm/ZerO_initialization.tex <==

% \begin{algorithm}[h]
% \caption{
%     \emph{\textit{ZerO Initialization for ResNet.}}
% }
% \begin{spacing}{1.15}
% \begin{algorithmic}
% % \State {\bfseries Input: } 
% \State {\bfseries Step 1.} \textbf{Add additional residual connections to ResNet} (Figure \ref{fig:structure})
% \State {\bfseries Step 2.} \textbf{Apply Hadamard transform to dimension-increasing residual connections} (Figure \ref{fig:resnet_special})
% \State {\bfseries Step 3.} \textbf{Initialize both first convolutional layer and the last classification layer to zero.}
% \State {\bfseries Step 4.} \textbf{Initialize residual blocks to zero and one.}
% % % \State {\bfseries Step 2. } $c_{min} \gets min(c_{in},c_{out})$
% % \State {\bfseries Step 3. } For $i = 0,...,c_{min}-1$, initialize $K[0,0,i,i] \gets 1$
% % \State {\bfseries Return } $K$
% \end{algorithmic}
% \end{spacing}
% \label{alg:zero_init}
% \end{algorithm}


% \newtcolorbox{mybox}[2][]{fonttitle=\bfseries,enhanced,attach boxed title to top center={yshift=-2mm},title={#2},#1}

\newtcolorbox{mybox}[2][]{%
    colback=cyan!5!white,
    colframe=cyan!75!black,
    fonttitle=\bfseries,
    enhanced,
    center title,
    colbacktitle=cyan!85!black,
    title={#2},#1}

\begin{mybox}{ZerO Initialization for ResNet}
\begin{enumerate}
    \item \textbf{Add additional residual connections.}
    \item \textbf{Initialize dimension-increasing residual connections as Hadamard transform.} 
    \item \textbf{Initialize residual blocks to zero and one.}
    \item \textbf{Initialize both the first convolutional layer and last classification layer to zero.}
\end{enumerate}
\label{alg:zero_init}
\end{mybox}

==> algorithm/partial_identity.tex <==
\begin{algorithm}[h]
\caption{
    \textit{Partial-Identity Initializer} for $1\times1$ convolutional kernel.
}
\begin{algorithmic}

\State {\bfseries Input: } a $1 \times 1 \times c_{in} \times c_{out}$ convolutional kernel $K$, $c_{in}$ number of input channels, $c_{out}$ number of output channels.
\State {\bfseries Step 1. } For $i= 0,...,c_{in}-1$ and $j= 0,...,c_{out}-1$, initialize $K[0,0,i,j] \gets 0$
\State {\bfseries Step 2. } $c_{min} \gets min(c_{in},c_{out})$
\State {\bfseries Step 3. } For $i = 0,...,c_{min}-1$, initialize $K[0,0,i,i] \gets 1$
\State {\bfseries Return } $K$
\end{algorithmic}
\label{alg:partial_identity}
\end{algorithm}


% \item[\textbf{Optimization parameters:}]
%     learning rate $\eta$;
%     averaging constant $\beta$;
%     weight clipping $\sigma^*$.
% \State $\bar{g} \gets 0$
% \Repeat
%     \State $g\gets \mathrm{StochasticGradient()}$ 
%     \State $\bar{g}^2 \gets (1-\beta) g^2 + \beta \bar{g}^2$                    
%     \State $W \gets W \odot \exp [-\eta \, \sign (W) \odot \clamp(g/\bar{g})]$
%     \State $W \gets \clamp_{\sigma^*} (W)$
% \Until{converged}
% \end{algorithmic}
% \label{alg:madam}
% \end{algorithm}

==> figures/breaking_rank_wrap.tex <==
\begin{figure}[t!]
    \centering
    \vskip -0.3in
    \includegraphics[width=0.9\textwidth]{figures/breaking_rank_constraint.pdf}
    \vskip -0.13in
    \caption{\small{\textit{Verify that the orthogonal transform breaks the rank constraint. We use the same setting in Figure~\ref{fig:rank_constraint} and focus on the matrix $\mW_{2}$ as a proxy. For some settings, we apply Relu as the nonlinearity or apply orthogonal transform to each layer. We also include the randomly initialized network for the comparison. \textbf{Left:} we measure the rank of the matrix $\mW_{2}$. \textbf{Right:} we measure the stable rank, which is defined as $\left\lVert \mW \right\rVert^{2}_{F} / \left\lVert \mW \right\rVert^{2}_{2}$ for any matrix $\mW$.}}}
    \label{fig:breaking_rank}
    \vskip -0.25in
\end{figure}

==> figures/linear_results.tex <==
\begin{figure}[t!]
    \centering
    \vskip -0.3in
    \begin{minipage}{0.5\textwidth}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/weight_distribution.pdf}
    \end{minipage}%
    \begin{minipage}{0.5\textwidth}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/correlation.pdf}
    \end{minipage}
    \vskip -0.13in
    \caption{\textbf{Left:} final weight distributions. \textbf{Right:} weight correlations during training. Each setting achieves 98\% test accuracy on MNIST dataset except for ZerO Init (no transform). }
    \label{fig:linear_results}
    \vskip -0.15in
\end{figure}

==> figures/lottery_ticket_results_wrap.tex <==
\begin{figure}[h!]
    \centering
    % \vskip -0.3in
    \begin{minipage}{0.3\textwidth}
    \centering
    \includegraphics[width=0.8\textwidth]{example-image-a}
    \end{minipage}%
    \begin{minipage}{0.3\textwidth}
    \centering
    \includegraphics[width=0.8\textwidth]{example-image-a}
    \end{minipage}
    \begin{minipage}{0.3\textwidth}
    \centering
    \includegraphics[width=0.8\textwidth]{example-image-a}
    \end{minipage}
    % \vskip -0.13in
    \caption{Lottery ticket results. \textbf{Left:} \textbf{Middle:} \textbf{Right:} }
    \label{fig:lottery_ticket}
    % \vskip -0.15in
\end{figure}

==> figures/low-rank_wrap.tex <==
\begin{figure}[h]
    \centering
    % \vskip -0.3in
    \begin{minipage}{.5\textwidth}
        \centering
        \includegraphics[width=0.8\linewidth]{figures/global_tucker2_resnet18.pdf}
    \end{minipage}%
    \begin{minipage}{.5\textwidth}
        \centering
        \includegraphics[width=0.8\linewidth]{figures/local_512_tucker2_resnet18.pdf}
    \end{minipage}
    % \vskip -0.13in
    \caption{\small{\textbf{Left:} a global Tucker-2 decomposition performed over all convolutions in ResNet-18. \textbf{Right:} a local Tucker-2 decomposition for a particular convolution with 512 channels in ResNet-18.}}
    \label{fig:low_rank_wrap}
    % \vskip -0.15in
\end{figure}

==> figures/rank_constraint_verification_wrap.tex <==
\begin{figure}[t!]
    \centering
    \vskip -0.3in
    \includegraphics[width=0.9\textwidth]{figures/rank_constraint_verification.pdf}
    \vskip -0.13in
    \caption{\small{\textit{Verify the rank constraint in Theorem~\ref{thm:low_rank_gd} on MNIST. The red dash line denotes $\max (n_x,n_y) = 784$. Consider a deep linear network $\funcF(\vx) = (\mW_{L} +\mI_{L}) \prod_{i \in \{2,...,L-1 \}} (\mW_{i} + \mI) (\mW_{1} + \mI_{1}) \vx$, where $\mW_{i} \in \sR^{n_h \times n_h}$, $\mW_{L}, \mI_{L} \in \sR^{n_y \times n_h}$, and $\mW_{1}, \mI_{1} \in \sR^{n_h \times n_x}$. We set $L=6$ in the experiment. \textbf{Left:} the matrix rank is independent of the hidden dimension $n_h$. We measure the rank of $\mW^{2}$ given various widths $n_h$. \textbf{Right:} the constraint holds for any matrix in the network. Given a fixed width $n_h=2048$, we measure the matrix rank for each hidden matrix. To be noted, random initialization achieves maximum rank for each matrix through the entire training, as illustrated in Figure~\ref{fig:breaking_rank}.}}}
    \label{fig:rank_constraint}
    \vskip -0.15in
\end{figure}

==> figures/resnet_results.tex <==
% \begin{figure}[t!]
%     \centering
%     \vskip -0.3in
%     \begin{minipage}{0.5\textwidth}
%     \centering
%     \includegraphics[width=0.8\textwidth]{figures/convergence.pdf}
%     \end{minipage}
%     % \vskip -0.1in
%     \caption{\textbf{Left:} Convergence results. \textbf{Right:} Weight diversity over training.}
%     \label{fig:resnet_results}
%     \vskip -0.15in
% \end{figure}

% \setlength{\textfloatsep}{0.5pt}
\begin{wrapfigure}{R}{0.4\textwidth}
    \begin{minipage}{0.4\textwidth}
    \vskip -0.1in
    \centering
    \includegraphics[width=\textwidth]{figures/convergence.pdf}
    \end{minipage}
    \vskip -0.1in
    \caption{Training error over the first 5 epochs on ImageNet.}
    \label{fig:resnet_results}
    % \vskip -0.1in
\end{wrapfigure}

==> figures/resnt_special.tex <==
\begin{figure}[h!]
    \centering
    \vskip 0.25in
    \includegraphics[width=0.9\linewidth]{figures/resnet_special.pdf}
    \caption{\textbf{Left:} associated operations for each convolutional layer. \textbf{Right:} an illustration of a 1x1x3x5 partial-identity convolutional kernel.}
    \label{fig:resnet_special}
    \vskip -0.1in
\end{figure}


==> figures/strcutures.tex <==
\begin{figure}[h]
    \centering
    \vskip -0.1in
    \includegraphics[width=0.9\linewidth]{figures/structures.pdf}
    \caption{\textit{ZerO initialization for ResNet.} 
    We initialize the first and spatial-downsampling layers, which increase their channel dimensions, by columns of Hadamard matrices $\mH \mI^{*}$. We also add extra skip connections in each residual block. Here we omit Relu and batch normalization. See Figure \ref{fig:resnet_special} for a detailed design.}
    \label{fig:structure}
    \vskip -0.1in
\end{figure}

==> figures/symmetry_fig.tex <==
\begin{figure}[t!]
    \vskip -0.3in
    \centering
    \includegraphics[width=0.8\linewidth]{figures/symmetry.pdf}
    % \vskip -0.3in
    \caption{\textbf{Left:} the forward dynamic of the zero-initialized example network at initialization. Solid and dashed blue lines represent non-zero signals. \textbf{Right:} we represent the signals in the first layer at initialization on a standard 2-dimensional basis. Dashed lines represent the signals before the Relu and solid lines represent the signals after the Relu, which are activations $\vx^{1}$.
    }
    \label{fig:symmetry}
    \vskip -0.15in
\end{figure}

==> figures/weight_distribution_wrap.tex <==
\begin{figure}[t!]
    \centering
    % \vskip -0.3in
    \includegraphics[width=0.4\textwidth]{figures/weight_distribution.pdf}
    % \vskip -0.13in
    \caption{Final weight distributions on MNIST}
    \label{fig:weight_distribution}
    % \vskip -0.15in
\end{figure}

==> sections/2-intro-old.tex <==
\section{Introduction}

% deep learning goods and it depends on random weight initialization
Deep learning applications have been widely used in recent years. An important question of training a deep neural network is how to initialize its weights. When \citet{<first_backward>} introduced backward propagation, they initialize neural networks randomly to break symmetries between parameters and neurons. Nowadays, random weight initialization is a common practice across various architectures and tasks. 

However, it is well known that the choice of random initialization methods significantly affects the quality of training. This is because random initialization inevitably requires prior knowledge on weight variance, such as predefining a standard deviation for a zero-mean Gaussian distribution, which is used to generate random weights. A random initialization scheme with inappropriate initial weight variance leads to signal vanishing or exploding, and thus fails the entire training. Popular initialization schemes like Xavier and Kaiming are designed by ensuring that the variance of the signals does not grow exponentially with depth at initialization \citep{<kaiming>,<xavier>}. Still, those methods highly depend on network architectures and are hard to be generalized. Various random initialization schemes are therefore designed to accommodate different architecture settings \citep{<fixup>,pennington_resurrecting_2017,saxe_exact_2014,mishkin_all_2016}. 

% many initialization, different initialization affects the accuracy. variance is one of the only problem. don't talk variance too explicitly 
% for xavier initialization, use citation instead of xavier initialization
% drop the last second sentence
% generalize this setting. 

% add something like: 
% introduce variance problem first , then talk about how to solve it (controlling weight variance different)

A natural idea to replace random initialization is initializing all the weights to zero, as it does not require any consideration of weight variance. However, zero initialization usually involves dead neuron problem where the weights associated with a neuron stop updating values due to zero derivatives.

% introduce residual network
% residual network solves derivatives, constant signals 
% too big, blow up. to small, vanishing
% some skip connections prevent signal vanishing 
% However, they still need some random initialization because skip connections not everywhere 


% Then next paragraph we talk about for modern architurectures   

Although fully zero-initialized neural networks are far from standard practice, zero-initialized weights start to play an important role in newly developed initialization methods. When initializing residual networks, recent studies suggest that signal propagation benefits from initializing a part of weights as zero. As studied in \citet{<mean_field>}, signal propagation is optimized when the entire signal only passes through the residual connections at initialization, which nearly forms the residual network as an identity mapping. To achieve this, a direct solution is initializing a few weights in the residual branches as zero to block the signals. For example, \citet{<rezero>} devise a zero-initialized scale factor $\alpha$ to every residual branch, such as: $x + \alpha \, F(x)$ where $x$ is the input and $F$ is a residual function. 

Initializing residual branches around zero also enables training residual networks without normalization. \citet{<skipinit>} suggests that batch normalization biases residual blocks towards identity functions at initialization. Since it is aligned with the aforementioned conditions for achieving the optimal signal propagation, this finding explains why batch normalization enables stable training and fast convergence. To train residual networks without normalization, for example, \citet{<fixup>} initialize the last layer in every residual branch to zero, which also forms the residual network as nearly an identity mapping.

Despite the effectiveness when partially initializing weights to zero, none of the previous initialization schemes achieves a fully zero-initialized setting, as zero initializing two consecutive layers causes zero derivatives. Still, the success of initialization with partial zero weights sheds light on designing a fully zero-initialized residual network.
% use dynamical isometry instead of \citep{mean_field}

In this work, we challenge widely used random weight initialization by proposing a \textit{fully deterministic initialization} called ZerO. ZerO initializes residual networks with only \textit{zeros and ones}. Surprisingly, such a simple initialization achieves state-of-the-art performances over various tasks and network structures. 

\textbf{Our contributions are summarized as follows:}
\begin{enumerate}[leftmargin=*]
    \item We carefully identify training difficulties that occurred when initializing residual networks to zero, which includes dead neurons and learning symmetries. We also address those difficulties by utilizing residual connections and applying Hadamard transform, respectively.
    \item We propose ZerO initialization, which takes zero-initialized weights to the extreme while using a few one-initialized weights to ensure stable signal propagation. With minor structure modifications, our ResNet-50 achieves 76.3\% accuracy on ImageNet when initializing 99.9\% weights to zero and 0.1\% weights to one.
    \item We apply ZerO to normalization-free residual networks and find that ZerO with proper regularization matches batch normalization baseline and other normalization-free techniques.
\end{enumerate}



% use linear model as an example and mention sample diversity

% option: random features, learning symmetries 
% Many works indicate that feature diversity from both sample diversity and random weight initialization are important for training. Few works are discussing how large the feature diversity should be. Can we solely rely on sample diversity (should consider the name)? 

% option: optimization view, close to global solution

==> sections/4-theory-1-x.tex <==
\section{Why does a zero-initialized neural network work?}
\label{sec:zero_init}

In this section, we discuss why a zero-initialized neural network should work and why residual networks are the preferred candidates. We wish to train the function $\funcF(\vx)$ to learn a particular input-output map given a set of $P$ training samples $(\vx^{\mu},\vy^{\mu}) \in \sR^{n_x \times n_y}$, where $\mu = 1,...,P$. 
Training is accomplished by minimizing the squared error $\loss = \frac{1}{2} \sum_{\mu=1}^{P} \norm{\vy^{\mu} - \funcF(\vx^{\mu})}_2^2$ using gradient descent with a step size $\eta$.

% change layer dimension notation from P,Q to N_l,N_r.
We model $\funcF(\vx)$ to be a multilayer perceptron with $L$ hidden layers: $\funcF(\vx) =  \phi(\mW_{L}) \circ ... \circ \phi(\mW_{1}) \circ \vx$, where $\circ$ is composition operator, $\mW_{l} \in \sR^{n_h \times n_h}$ for $l \in 1,...,L$. $n_h$ denotes a unified hidden dimension and $\phi$ represents an identity function or an nonlinearity. 
% Note the change: we change layer activation a^{1} to a^{1}. Remember to change everywhere.
% We ignore bias terms, and denote $\va^{l} = \phi(W^{l} \, \va^{l-1})$ as the activations of the $l$th layer, where $\va^{0} = \vx$.
% We also define $\mW^{l}_{i,:}$ and $\mW^{l}_{:,j}$ to be $i$th row and $j$th column of the matrix $\mW^{l}$.

\subsection{Zero initialization is data-dependent}

% Linear Case Warmup (could be a new warmup section)
We first consider a simple linear case to illustrate why zero initial weights should work. 
Let $\funcF(\vx) = \mW \vx$ and assume $\funcF$ has the uniform dimensionality: $n_x = n_y = n_h$. We train the function using gradient descent with a step size of $\eta$. 
The derivative of the initial matrix $\mW_0$ at zero becomes:
\begin{equation}
    \label{eq:init_non_zero_sol_plain}
    \grad{\loss}{\mW_0} = - \sum_{\mu=1}^{P} \vy^{\mu} \vx^{\mu^{T}} = - \Sigma_{\vy \vx},
\end{equation}
where $\Sigma_{\vy \vx} = \sum_{\mu=1}^{P} \vy^{\mu} \vx^{\mu^{T}}$ denotes the  input-output correlation matrix. 
The matrix $\mW_1$ at the first step becomes:
\begin{equation}
    \mW_1 = \mW_0 - \eta \grad{\loss}{\mW_0} = \eta \Sigma_{\vy \vx}.
\end{equation}
As shown above, when initializing $\mW_0$ at zero, the first non-zero matrix $\mW_1$ updated through gradient descent becomes a $\eta$-weighted input-output correlation matrix. 
Unlike random initialization independent of the underlying samples, zero initialization forms an initial non-zero solution solely depending on the samples themselves. 
We call that zero initialization is a \textit{data-dependent initialization}. This property plays an important role in our following analysis.

% A special case when inputs are orthogonal: the derivative and the weight matrix are formed by \Sigma_{\vy \vx} through training. It becomes an univariate optimization problem. (might mention in appendix)
% We also denote $\Sigma_{\vx \vx} = \sum_{\mu=1}^{P} \vx^{\mu} \vx^{\mu^{T}}$ as the input-input correlation matrix. To simplify the analysis, we assume that input representations are orthogonal, such that $\Sigma_{\vx \vx} = I$. This assumption can be easily achieved by the whitening transform used in data preprocessing.

Now we extend to a linear multilayer perceptron with $L$ hidden layers: $\funcF(\vx) = \mW_{L} \mW_{L-1} ... \mW_{1} \vx$, where $l \in 1,...,L$ and $L \ge 2$. 
We assume the origin is not a local minimum, which happens almost surely in practice. 
Therefore, the origin becomes a saddle point in the loss landscape, where the derivative of any matrix $\mW_{l}$ is zero. 
Under this setting, zero initialization stalls at the saddle point, and no weights can move out of the zero during the entire training. 
This is also a special case of the well-known \textit{dead neuron problem}, where all neurons consistently output zero values.

% To address this problem, we equip $\funcF$ with skip connections, which reshapes the loss landscape and thus avoid the saddle point at zero.

\subsection{Skip connections avoid saddle property at zero}
% For simplicity, we first assume that $\funcF(\vx)$ is a linear network with a fixed dimension, such that $n_x = n_y = N_{l}^{l} = N_{r}^{l}$ for any $l$, and $\phi$ is an identity mapping. In this case, if we initialize the weights to zero, every layer will output zero constantly no matter what the inputs are. On the other hand, every $\mW^{l}$ receives zero derivatives in the backward pass, and thus there is no weight that can move out of the zero during the entire training. This extreme case of the vanishing gradient problem, well-known under the name \emph{dead neuron problem}, is caused by zero-initialized $\funcF(\vx)$ only generating zero signals at initialization. 

The reason behind the dead neuron problem is that the derivative of each matrix $\grad{\loss}{\mW^l}$ solely depends on a high-order factor, which consists of the rest of the matrices. 
For example, consider $\funcF(x) = w_L ... w_1 x$ for scalar parameters $w_1, ... ,w_L \in \sR$. The derivative of any parameter $\grad{\loss}{w_i}$ only depends on a high-order factor $\prod_{j\neq i}^{L} w_j$, which is the product of the rest of the parameters.
The deeper the function becomes, the higher the order of the factor is. 
This makes the origin becomes a highly degenerated saddle point. 

To remove the critical point at the origin, it is necessary to employ a low-order factor in each derivative, which does not depend on other parameters. 
The low-order factors can be included by equipping every layer in $\funcF$ with a skip connection. 
% Skip connections help propagate signals through the network and thus mitigate the vanishing gradient problem. 
% A natural approach towards practical zero initialization is therefore to equip \emph{every} layers of the network with skip connections. 
% This ensures that the signal is propagated even with zero weights, with each layer applying a simple identity function to the activations. 
This forms $\funcF$ to become a residual network:
\begin{equation}
    \label{eq:fixed_dim_linear_residual}
    \funcF(\vx) = (\mW_{L} + \mI) ... (\mW_{1} + \mI) \vx.
\end{equation}
where $I$ is an identity function. When initializing each $\mW^{0}_{l}$ at zero, the initial derivatives become:
\begin{equation}
    \label{eq:gradient_at_zero_dim_fixed_residual}
    \grad{\loss}{\mW^{0}_{l}} = \Sigma_{\vx \vx} - \Sigma_{\vy \vx} \quad \text{for } l \in 1,...,L,
\end{equation}
% left for further explanation
% The derivatives with respect to weight matrices are then given as
% \begin{equation*}
%     \begin{split}
%         \grad{\loss}{\mW^1} &= ((\mW^L + \mI) \,...\, (\mW^2 + \mI))^{T} \, (\hat{y} - y) \, \vx^{T}, \\
%         %to-do think about whether we should exclude l=2 and l=L-1 as well
%         \grad{\loss}{\mW^l} &= ((\mW^L + \mI) \,...\, (\mW^{l+1} + \mI))^{T} \, (\hat{y} - y) \, ((\mW^{l-1} + \mI) \,...\, (\mW^{1} + \mI) \, \vx)^{T} \quad \text{for } l \in 2,...,L-1, \\
%         \grad{\loss}{\mW^L} &= (\hat{y} - y) \, ((\mW^{L-1} + \mI) \,...\, (\mW^{1} + \mI) \, \vx)^{T}.
%     \end{split}
% \end{equation*}
where $\Sigma_{\vx \vx}$ is the input-input correlation matrix. Because $(\Sigma_{\vx \vx} - \Sigma_{\vy \vx})$ is a non-zero low-order factor not depending on other matrices, the origin is no longer a critical point. After the first weight update, every matrix uniformly becomes:
\begin{equation}
    \label{eq:init_non_zero_sol}
    \mW^{1}_{l} = \eta (\Sigma_{\vy \vx} - \Sigma_{\vx \vx}) \quad \text{for } l \in 1,...,L.
\end{equation}
Compared to Equation~\ref{eq:init_non_zero_sol_plain}, $\mW^{1}_{l}$ in Equation~\ref{eq:init_non_zero_sol} additionally depends on the input-input correlation matrix due to the residual structure. 
In addition, Equation~\ref{eq:init_non_zero_sol} indicates that zero initialization is still data-dependent under any arbitrary deep residual network. 

In Equation~\ref{eq:init_non_zero_sol}, all weight matrices $\mW^{0}_{l}$ receive the same derivatives.
However, as the training progresses, the high-order factors in the derivatives become significant, and thus the overall derivatives become distinct for $\mW^{0}_{l}$ at different positions in the network.

We note that zero initialization also works for residual networks with nonlinearity, if and only if the derivative of the nonlinearity exists at zero. For nonlinearities not satisfying this condition, such as Relu \citep{xu_empirical_2015}, this can be solved by propagating one of its subderivatives at zero during backpropagation \footnote{In our experiments, we propagate $\phi^{\prime}(0) = 1$ for Relu, which allows the signals to be identically propagated.}. 

% to-do: mention that SGD is slower than GD (could put to the rank part with experiments)

% Not mention symmetry
% We note that the network inputs serve not only as non-zero signals propagated at initialization but as important symmetry breakers that decouple the weight correlations at initialization. It is well known that initializing the weights using the same value may cause symmetries between parameters and neurons, which damages the expressiveness of the network. 

% In addition, in our setting every weight matrix receives the same derivatives $(\vy - \vx) \, \vx^{T}$, which causes the symmetries between matrices at initialization. However, the symmetries between them are decoupled during training due to the depth difference. 

Zero initialization under linear residual networks is also called \textit{identity initialization}, as the input is identically propagated to the output at initialization. 
From an optimization perspective, identity initialization has been well studied through both landscape-based and trajectory-based methods. 

\citet{hardt_identity_2016} suggests that for linear residual networks, there exists a global minimum that is very close to the origin, such that: $\max_{1 \leq l \leq L} \left\lVert \mW^{*}_{l} \right\rVert \leq O(1/L)$ for large enough $L$, where $\left\lVert \mW \right\rVert$ denotes a spectral norm. 

In terms of the rate of convergence, \citet{bartlett_gradient_2019} proves that under identity initialization, gradient descent learns an $\epsilon$-approximation of $\funcF$ within iterations polynomial in $log(1 / \epsilon)$, given that the loss at the origin is not too large. 
% to-do: may add another one regarding better step size

These results indicate that for deep linear residual networks, zero initialization is not only guaranteed to converge but also to be a good initial guess close to the global minimum. 
However, in practice, none of the previous works achieve the exact zero initialization (without small random perturbations). 
This is mainly because of the dimension-varied compositions and complex operations in modern residual networks.
We will describe these problems later and propose solutions to address them.


==> sections/4-theory-2-x.tex <==
\section{Zero initialization leads to rank-constrained solutions}
\label{sec:zero_rank_constraint}
% \subsection{Zero initialization leads to rank-constrained solutions}

%\input{figures/symmetry_fig}
The deep linear residual networks discussed above have a uniform dimensionality across the input, output, and hidden layers. However, for modern residual networks, the hidden dimensions are usually larger than the input and output dimensions. 
In this case, under zero initialization, we find that gradient descent only converges to a rank-constrained solution, where the constraint only depends on the input and output dimensions, no matter how large the hidden dimensions are. 

To explain our finding, we assume the linear residual function defined in Equation~\ref{eq:fixed_dim_linear_residual} has arbitrary hidden dimension $n_h$, where $n_h$ may be different from $n_x$ and $n_y$. To let the skip connections connect two layers with different dimensions, we define \textit{adaptive identity mapping}, which maximally preserves the input information to the output.
\begin{definition}
    Let $\mI^{*} \in \sR^{l \times r}$ where $l \neq r$. We call $\mI^{*}$ an adaptive identity mapping if for any input vector $\vx = (x_1,x_2,...,x_{r})$, it satisfies:
    \begin{equation}
        \label{eq:adaptive_identity}
        \mI^{*}(\vx) = 
        \begin{cases}
            (x_1,x_2,...,x_{l}) & \text{if } l < r, \\
            (x_1,x_2,...,x_{r},\underbrace{0,...,0}_{l-r} ) & \text{otherwise.}
        \end{cases}
    \end{equation}
\end{definition}
According to the definition, the adaptive identity mapping clips the last few dimensions when shrinking the space, and it pads additional dimensions with zero when expanding the space. 
In practice, these are standard parameter-free techniques used for connecting dimension-varied layers, such as channel-expanding layers in ResNet \citep{resnet}.

To simplify our analysis, we limit our focus on linear residual networks with a uniform hidden dimensionality $n_h$. The complete definition is provided below:
\begin{definition}
\label{def:linear_residual_network}
    Consider a linear residual network $\funcF(\vx) = (\mW_{L} + \mI_{L}) ... (\mW_{2} + \mI) (\mW_{1} + \mI_{1}) \vx$ with $L \geq 2$. Let $\mW_{L},\mI_{L} \in \sR^{n_y \times n_h}$ and $\mW_{1},\mI_{1} \in \sR^{n_h \times n_x}$, where $\mI_{L}$ and $\mI_{1}$ are adaptive identity mappings defined in Equation~\ref{eq:adaptive_identity}. For any layer $l$ except $1$ and $L$, we assume $\mW_{l} \in \sR^{n_h \times n_h}$ and we let $I \in \sR^{n_h \times n_h}$ to be the standard identity mapping.
\end{definition}

Given everything we need, we present our main theorem as follows:
\begin{restatable}{theorem}{low_rank_gd}
    \label{thm:low_rank_gd}
    Consider a linear residual network defined in Definition~\ref{def:linear_residual_network}. When initializing every matrix $W_{l}$ at zero and training the function using gradient descent, at any iteration $t$, we have that:
    \begin{equation*}
        \rank(W_{l}^{t}) \leq \min (n_x, n_y) \quad \text{for } l \in 1,...,L.
    \end{equation*}
\end{restatable}

We provide a sketch of the proof here and present the detailed proof in the appendix. We focus on the case of large hidden dimension $n_h > n_x,n_y$ as it is non-trivial. In this case, for each matrix $W_{l}$, the gradient descent only updates the weights over a \textit{low-dimensional subspace} with a maximum size of $n_x \times n_y$. This is because the rest of the space stalls at a saddle point, even at the beginning. 

To see this, we need to expand out analysis of the initial derivatives in Equation~\ref{eq:gradient_at_zero_dim_fixed_residual} from a uniform dimension setting to ours, which is stated below:

\begin{lemma}
    \label{lemma:init_gradient}
    Consider a linear residual network defined in Definition~\ref{def:linear_residual_network}. When initializing every matrix $W_{l}$ at zero and training the function using gradient descent, at the beginning, we have that:
    \begin{equation*}
        \begin{split}
            \grad{\loss}{\mW_{1}^{0}} &= \mI_{L}^{\top} (\mI_{L} \mI_{1} \Sigma_{\vx \vx} - \Sigma_{\vy \vx}), \\
            \grad{\loss}{\mW_{l}^{0}} &= \mI_{L}^{\top} (\mI_{L} \mI_{1} \Sigma_{\vx \vx} - \Sigma_{\vy \vx}) \mI_{1}^{\top} \quad \text{for   } l \in 2,...,L-1, \\
            \grad{\loss}{\mW_{L}^{0}} &= (\mI_{L} \mI_{1} \Sigma_{\vx \vx} - \Sigma_{\vy \vx}) \mI_{1}^{\top}.
        \end{split}
    \end{equation*}
\end{lemma}
As shown in Lemma \ref{lemma:init_gradient}, zero initialization is still fully data-dependent as $\mI_{1}$ and $\mI_{L}$ are deterministic operators. In the following, we explicitly present the derivatives under the regime of large hidden dimensionality: 
\begin{lemma}
    \label{lemma:init_gradient_large_width}
    When $n_h > n_x,n_y$, the initial derivatives become:
    \begin{equation*}
    \grad{\loss}{\mW_{1}^0} = 
    \begin{pmatrix*}
        \Lambda \\
        \bm{0} \\
    \end{pmatrix*}
    \in \sR^{n_h \times n_x},
    \quad
    \grad{\loss}{\mW_{l}^0} = 
    \begin{pmatrix*}
        \Lambda & \bm{0} \\
        \bm{0} & \bm{0} \\
    \end{pmatrix*}
    \in \sR^{n_h \times n_h},
    \quad
    \grad{\loss}{\mW_{L}^0} =
    \begin{pmatrix*}
        \Lambda & \bm{0} \\
    \end{pmatrix*}
    \in \sR^{n_y \times n_h},
    \end{equation*}
    where $\Lambda = \mI_{L} \mI_{1} \Sigma_{\vx \vx} - \Sigma_{\vy \vx} \in \sR^{n_y \times n_x}$ and $l \in 2,...,L-1$. We denote $\bm{0}$ as a zero vector or a zero matrix depending on the dimensionality.
\end{lemma}

Lemma~\ref{lemma:init_gradient_large_width} suggests that in the initial derivative of each matrix, the elements are zero except for a sub-matrix determined by $\Lambda$. Further derivation indicates that the parameters with zero initial derivatives stall at zero during the entire training. 

% close the statement of theorem 1 
Because there is only a sub-matrix of $n_y \times n_x$ being optimized during training, the maximum rank of the each matrix is at most $\min (n_x, n_y)$. Thus, Theorem~\ref{thm:low_rank_gd} holds under the large hidden dimension condition $n_h > n_x, n_y$.  The theorem under other conditions can be proved in a similar way.

% validation 1: description of empirical evaluation: 3D plotting
% figure 1.a, 3D plotting visualizes the above setting

% validation 2: measuring the rank of the matrix under MNIST dataset
% figure 2.a, the rank is upper bounded by $n_x, n_y$

% empirical verification
We empirically verify the above result by training the network on MNIST. As shown in Figure~\ref{fig:rank_constraint}, the rank constraint holds for every matrix no matter how large the hidden dimension is or how many training iterations are performed.

% explain from optimization point of view
% to-do: change to more formal math statement
We continue our discussion under $n_h > n_x, n_y$. From an optimization viewpoint, \textit{the converged low-rank solution is a saddle point over the entire parameter space}.
Assume $\mV$ is the vector space of all parameters in $\funcF$. Let $\mK \in \sR^{L \times n_x \times n_y}$ to be a subspace of $\mV$, which has initial derivatives determined by $\Lambda$. Let $\mM$ to be the rest space with zero initial derivatives. 
The gradient descent only searches the solution over $\mK$ during training as $\mM$ gets stuck at zero. Thus, even gradient descent converges to a minima in $\mK$, it is merely a saddle point over the entire parameter space $\mV$.

% consider to comment out this paragraph to reduce confusion
% We note that Theorem~\ref{thm:low_rank_gd} is not because each hidden layer only has $n_x$ active dimensions while other $n_h - n_x$ dimensions stay at zero. 
% In fact, Theorem~\ref{thm:low_rank_gd} also holds if we apply orthogonal transforms to ensure no constant zero dimensions in each hidden layer. 
% For example, we apply an orthogonal transform $\mO \in \sR^{n_h \times n_h}$ after expanding the dimension from $n_x$ to $n_h$, such that $\funcF(\vx) = (\mW^{L} + \mI^{L}) \mO^{\top} ... (\mW^{2} + \mI) \mO (\mW^{1} + \mI^{1})$. 
% In this case, no hidden layer receives zero input signals but the low-rank constraint still holds because zero elements are persisted in the derivative wrt. each matrix. 
% to-do: figure 2, empirical verification with orthogonal transform

The low-rank constraint restricts the expressivity of the linear residual network $\funcF$, and thus the training only converges into a \textit{underfitting regime} for complex learning tasks. To make the zero initialization work in practice, we need to break the low-rank constraint during training.

\input{figures/rank_constraint_verification_wrap.tex}

% put in the structure section (old)
% For popular convolutional residual networks, their computational logic usually follows expansions of channel dimension and reductions of spatial dimension. For example, ResNet-18 proposed by \citep{resnet} expands the channel dimension from 3 to 512 while reducing thehe first weight updates, the columns of spatial dimension to 1 for each channel in the end. When applying skip connections to channel expanding layers, a standard non-parametric method is duplicating all channels from the previous layer while padding additional channels as zero, which is also called constant padding skip connection.

\subsection{Hadamard transform breaks the rank constraint}

% new section: solutions
% optional: mentioning saddle to saddle dynamics, we actually accept saddle to saddle dynamics from the lowest rank to middle rank. However, small random perturbation is required to escape the saddle point using GD.

% We want to push it further to keep our extreme zero and deterministic initialization. Randomness is not allowed in our design principle. Thus, we break the saddle point by utilizing non-linearity.
% still need to figure out how to motivate the non-linearity part.
% Non-linearity helps to reshape the loss landscape and thus to break the saddle point. However, zero is special case that not works (hard to expand to why but it is necessary). Then saying Hadamard transform maximumly rotates the sapce to disentangle from the space based on standard basis (weakly aligned argument); finally, show how rank goes with these treatments; Comments on the slow rank growing trajectory of zero initialization.

% low-dimension subspace, need to apply a transformation to spread it over a new space
% Hadamard transform can spread it maximumly 

We move our focus to nonlinear networks widely used in practice. Nonlinearity increases the network expressivity as it decouples the linear dependency and thus increases the overall rank. However, we show later that the nonlinearity does not work under a particular condition that happened in zero initialization. We instead propose to use Hadamard transform to avoid such a condition.  

To simplify our explanation, we assume a single-layer residual network with varying dimensionality: $\funcF(\vx) = \mI_{2} (\mW + \mI) \mI_{1} \vx$, which has a large hidden space $n_h > n_x, n_y$. Let $\mW \in \sR^{n_h \times n_h}$, and $\mI_{1} \in \sR^{n_h \times n_x}$ and $\mI_{2} \in \sR^{n_y \times n_h}$ to be adaptive identity mappings. When initializing $\funcF$ at zero, it still holds the rank constraint in Theorem~\ref{thm:low_rank_gd}. Our objective is to ensure $\rank (W^t) > \min (n_x, n_y)$ happens at a iteration $t$ during training.

% to-do: check if the equation here is correct. 
First we add nonlinearity to the function, such that: $\funcF(\vx) = \mI_{2} \circ \phi \circ (\mW + \mI) \mI_{1} \vx$, where $\phi$ is an element-wise nonlinearity. The derivative at zero becomes:
\begin{equation}
    \grad{\loss}{\mW^0} = \sum_{\mu=1}^{P} \phi^{\prime}(\mI_{1} \vx^{\mu}) \odot \mI_{2}^{\top} (\mI_{2} \odot \phi (\mI_{1} \vx^{\mu}) - \vy^{\mu}) \vx^{\mu^{\top}} \mI_{1}^{\top},
\end{equation}
where $\odot$ is the element-wise multiplication. As shown in the above equation, $\mI_{1}$ maps $x^{\mu}$ into a low-dimensional subspace with the size of $n_x$. After applying the nonlinearity, $\phi (\mI_{1} \vx^{\mu})$ stays in this subspace as $(\mI_{1} \vx^{\mu})_i = 0$ for any $i > n_x$. In other words, the linear dimension of $\mI_{1} \vx^{\mu}$ is invariant under application of any nonlinearity $\phi$ because it lives in a subspace with $n_h - n_x$ dimensions aligned with each other over the standard basis. This is the reason why nonlinearity can not expand the dimensionality under zero initialization.

To expand the dimension using $\phi$, we need to disentangle the alignment between $n_h - n_x$ dimensions in $\mI_{1} \vx^{\mu}$. A natural way is applying an \textit{random orthogonal transform} $\mO \in \sR^{n_h \times n_h}$ over the hidden space, such that $\funcF(\vx) = \mI_{2} \mO^{\top} (\mW + \mI) \mO \mI_{1} \vx$. In this case, after feeding any $\vx^{\mu}$ into the hidden space, $\mO \mI_{1} \vx^{\mu}$ is no longer aligned with the standard basis for any dimension, almost surely. 

% to-do: follow our previous experiments showing how this works empirically.
In Figure~\ref{fig:breaking_rank}, we empirically verify that the random orthogonal transform breaks the rank constraint in non-linear residual networks. It also shows that both orthogonal transform and nonlinearity are necessary for breaking the rank constraint. We also measure \textit{stable rank}, which is defined as: $\left\lVert \mW \right\rVert^{2}_{F} / \left\lVert \mW \right\rVert^{2}_{2} = \sum_{i=1}^{k} \sigma^{2}_{i} (\mW) / \sigma^{2}_{max} (\mW)$ for any matrix $\mW$ with k singular values $\sigma_{i}$. Stable rank is a soft version of the operator rank, and unlike rank, it is less sensitive to the small singular values. 

Low stable rank indicates the imbalance between small and large singular values, which favors low-rank approximation. As suggested by \citet{sanyalStableRankNormalization2020}, reduicng the stable rank also improves the generalization. Figure~\ref{fig:breaking_rank} suggests that although the orthogonal transform breaks the rank constraint and improves the prediction performance, each matrix is still in a regime of low stable rank during training. This motivates us to discover the effect of low-rank approximation, where the zero-initialized networks could be approximated into a low-rank format while preserving the accuracy. 

% Hadamard transform 
To eliminate the randomness while relaxing the alignment, we pick a particular orthogonal transform called \textit{Hadamard transform}. The Hadamard transform rotates the standard basis into a new basis, such that each dimension in the new basis is \textit{equally weakly aligned} with every dimension over the standard basis. For example, in a two-dimensional space, the Hadamard transform rotates the standard basis by an angle of $45$ degree. 

We recap the definition and basic properties of Hadamard transform in the appendix. We pick the Hadamard transform because it not only maximally disentangles the alignment between the additional dimensions, but it is also memory and computationally efficient. The Hadamard transform consists of a Hadamard matrix and a constant normalization factor, where the Hadamard matrix contains $1$ and $-1$ only. Therefore, except for the scaling operation, it does not require any multiplication as sign flips are all it takes. It can be implemented efficiently with only $O(nlog(n))$ complexity \citep{fino_unified_1976}. 

We note that the Hadamard transform only needs to be applied to layers expanding the dimensionality for general deep neural networks. For example, in the ResNet structure proposed by \citet{resnet}, there are only a few types of channel dimension no matter how deep the network is. Thus, the Hadamard transform only needs to be applied at the layers increasing the channel dimension. 

\input{figures/breaking_rank_wrap.tex}
% option: mention how many percentage Hadamard transform increase the FLOPs


% \subsection{Measuring rank and weight distribution}
% \input{figures/linear_results}
% put weight distribution to model compression section

% \textbf{to be changed with rank verification experiments}

% To verify the phenomenon explained above empirically, we train a fully connected residual network on the MNIST dataset to check the existence of the degeneracy and measure the weight distribution \citep{lecun_gradient-based_1998}. 
% Our network has three layers with hidden dimensions larger than the input dimension. The details of our setting are introduced in the appendix.

% may discuss it - the effect of sample correlation
%We also observe that the random initialization methods achieve smaller correlations than ours. We believe this is because, in our setting, the weights inherit the correlations from the samples, as they solely depend on the sample diversity at initialization. Although the additional sample correlations do not affect the final accuracy, it is an interesting direction to discover the effect of these correlations during training, and we will investigate it in the future.

% weight distribution
% In addition, we measure the final weight distributions over various initialization methods. As shown in Figure \ref{fig:linear_results}, the weight variance generated by our initialization is significantly lower than the variances generated by randomized methods. 
% We believe that the fact that most of our weights are close to zero may help to train sparse neural networks with techniques such as weight pruning\citep{han_heep_2016}.

% point out where we need to initialize as one, for batch-norm layers


%Previous methods to break the symmetric: random weight initialization, dropout or GPU arithmetics

% Compare those methods based on the measurements


==> sections/5-structure-x.tex <==
\section{ZerO Initialization}
\label{sec:ZerO}

Motivated by our theoretical understanding, we propose ZerO to generalize our deterministic method in practice. Unlike a simple fully-connected network $\funcF$, practical networks are composed of different operations, such as convolution, skip connection, and batch-normalization \citep{resnet,batchnorm}. Although ZerO requires customized consideration for different networks due to various operations and dimensionalities, it always follows the general design principle mentioned above, which eases the difficulty of applying ZerO. In the following, as an example, we will show how to apply ZerO to the well-developed ResNet architectures in \citet{resnet}.
% to-do: add different treatments for different operations in the appendix

It is a natural direction to apply ZerO on ResNet architectures, as they usually have skip connections between residual blocks to allow the signals to easily propagate through the network. The skip connections ensure that the input flows through the residual blocks even when they are initialized at zero instead of the identity. However, the operations inside each residual block require more consideration as they are not connected by the skip connections. In addition, due to varying dimensionality (e.g., downsampling process) in ResNet, the Hadamard transforms need to be applied in some cases. 

To best flow the input data through every layer in the ResNet, we apply some modifications to the original structure, which are minimal and efficient. Before discussing them, we introduce how to apply ZerO to modify and initialize the ResNet in general:
\input{algorithm/ZerO_initialization}
\input{figures/strcutures.tex}
\paragraph{Residual block.}
We first focus on the design of the residual blocks, which is the core component of ResNet architectures. We adopt the pre-activation block design proposed by \citet{he_identity_2016}, where the identity mappings (without nonlinearity) are applied as the skip connections. 

We first consider modifying the basic block by using the skip connections to avoid the dead neuron problem. As the channel dimension is fixed within each basic block, we can directly apply identity mappings to every convolutional block, which contains a convolutional layer, Relu activation, and batch normalization. This is illustrated in Figure \ref{fig:structure}.

The bottleneck block proposed by \citet{resnet} is used to reduce the computational complexity when training deep models on large-scale datasets. The block consists of two 1x1 and one 3x3 convolutions where 1x1 convolutions are used to reduce and increase the input and output dimensions of the 3x3 convolution. Because the dimensions are varied within each bottleneck block, applying skip connection to every convolution leads to information loss. This is because the skip connection only can propagate a part of activations when applying it to a layer that reduces the channel dimension.

To address this problem, we only apply the skip connections between layers that share the same dimension. As illustrated in Figure \ref{fig:structure}, we keep the original skip connection between the first and the last 1x1 convolutions and only add another skip connection to the 3x3 one. This design can be viewed as building a residual layer inside another residual layer, which does not cause the information loss as we mentioned above. However, directly initializing all convolutions to zero is not applicable, as there is no skip connection between the first 1x1 convolution and the 3x3 convolution. 

\paragraph{Partial-identity initialization.}
To address this, we initialize each 1x1 convolution as a \emph{partial identity} matrix, as it can be viewed as a linear projection over the channel dimension. For a $1 \times 1 \times c_{in} \times c_{out}$ convolutional kernel $K$, where $c_{in}$ is the number of input channels and $c_{out}$ is the number of output channels. Initializing $K$ is equivalent to initializing a $c_{in} \times c_{out}$ matrix $\hat{K}$. As $c_{in}$ and $c_{out}$ may be different, we initialize the largest square matrix in $\hat{K}$ as identity matrix and initialize the rest components to zero. This is illustrated in Figure \ref{fig:resnet_special}. Specifically, let $c_{min}$ to be the minimum of $c_{in}$ and $c_{out}$, the matrix $\hat{K}$ is initialized as follows:
\begin{equation}
\label{eq:partial_identity}
\begin{split}
    \hat{K}_{i,i} &= 1 \quad \text{for } 0 \leq i \leq c_{min}-1, \\
    \hat{K}_{i,j} &= 0 \quad \text{for } 0 \leq i \leq c_{in}-1, 0 \leq j \leq c_{out}-1, \text{ and } j \neq i.
\end{split}
\end{equation}
When $c_{in} \leq c_{out}$, this essentially initializes the linear projection as an identity mapping with zero padding. This allows signals to be propagated through the layer while initializing the weights deterministically. Therefore, by initializing the first 1x1 convolution as a partial-identity matrix, the rest convolutions can be initialized to zero without damaging the signal propagation.
\input{figures/resnt_special}

\paragraph{Hadamard transform for dimension-increasing skip connections.}
Because the channel dimension is increased gradually in ResNet, there are various types of dimension-increasing skip connections developed, including simple identity mapping with zero padding and linear projection using 1x1 convolution. Although directly initializing 1x1 convolution to zero leads to zero signals, we can follow our previous design to initialize it as a partial-identity matrix, which also forms it as an identity mapping with zero padding. However, as discussed in Section \ref{sec:theory}, there is a training degeneracy when applying the zero padding operation during the width expansion. Therefore, we apply Hadamard transform for every dimension-increasing skip connection to solve the degeneracy, as illustrated in Figure \ref{fig:structure}.

In addition, depending on the channel dimension, we may apply a dimension-increasing skip connection and a Hadamard transform for the first convolution of the ResNet. For the last fully connected layer, we can safely initialize it to zero without any modification, as it receives both non-zero inputs and derivatives at initialization. For batch normalization layers, we initialize the scale as one and the bias as zero. For other operations in ResNet, such as average or max pooling, we keep them by default as they do not require any learnable parameters. 

% We note that applying Hadamard transforms does not introduce a significant overhead as the transform is computationally efficient. As defined at Definition \ref{def:hadamardmatrix}, a Hadamard matrix only consists of -1 and 1. Therefore, except for the scaling operation, it does not require any multiplication as sign flips are all it takes. It can be implemented efficiently with only $O(nlog(n))$ complexity \citep{fino_unified_1976}. 

% \paragraph{Training without batch normalization.}
% As motivated in the introduction, ZerO may help train neural networks without batch normalization, because both ZerO and batch normalization bias the residual network as an identity mapping at initialization. Therefore, we propose removing the batch normalization using learnable scalar multipliers and biases, which follows the design in \citep{<skipinit>,<fixup>}. This is illustrated in Figure \ref{fig:resnet_special}.

% to-do: a paragraph mentioning computational complexity

%  We note that our ZerO initialization shares similarities with some initialization schemes where they initialize a part of weights in the residual branch to zero, or initialize the last layer to zero \citep{<fixup>,<skipinit>,<rezero>}. However, they still require a substantial amount of random weights to propagate the signals and avoid the learning symmetries. We are the first to take the direction of zero and one initialization to the extreme. 

% Use subderivative one of Relu at zero, mentioned again.

==> sections/X-illustrations.tex <==
\section{Planning illustrations (Placeholders only)}

\subsection{Illustrating how orthogonal transformation breaks the symmetric}

\subsection{The structure of ZeroResNet}
\subsubsection{The design of normalization-free residual block}
\begin{figure}
    \centering
    \includegraphics[scale=0.3]{figures/basicblock.png}
    \caption{Zero Basic Block}
    % \label{fig:my_label}
\end{figure}
\subsubsection{Orthogonal transformation module}

\subsection{The initial dynamic of training}
\begin{figure}
    \centering
    \includegraphics[scale=0.3]{figures/training_dynamic1.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[scale=0.3]{figures/training_dynamic2.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

==> sections/X-method-discussion.tex <==
\section{Methodology Discussion}

\subsection{Modeling Assumption}
Consider the problem of learning a function $\loss(\vy, \funcF(\vx,\mW))$ using a set of $P$ training samples $\{\vx^\mu, \vy^\mu\}, \mu=1,...,P$. For dimensionality, $\vx \in \sR^{N_0}$, $\vy \in \sR^{N_L}$, and $\mW$ will be specified in the following cases individually. Training is accomplished via gradient descent on the squared error $\loss = \frac{1}{2} \sum_{\mu=1}^{P} \norm{\vy^{\mu} - \funcF(\vx^{\mu},\mW)}_2^2$.

\subsection{The simplest case: linear model}
Let's consider a linear model first: $\funcF(\vx,\mW) = \mW \vx$ where $\mW \in \sR^{N_L \times N_0}$. We ignore the bias term for simplicity. The derivative wrt. $\mW$ is: 
\begin{equation*}
    \frac{\partial \loss}{\partial \mW} = - \sum_{\mu=1}^{P}(\vy^{\mu} - \mW \vx^{\mu}) \vx^{\mu^\top} = \mW \Sigma^{11} - \Sigma^{31},
\end{equation*}
where $\Sigma^{11} = \sum_{\mu=1}^{P}\vx^{\mu} \vx^{\mu^\top}$ is an $N_0 \times N_0$ input correlation matrix, and $\Sigma^{31} = \sum_{\mu=1}^{P} \vy^{\mu} \vx^{\mu^\top}$is an $N_L \times N_0$ input-output correlation matrix.

We further assume the input has orthogonal representations where $\Sigma^{11} = \sum_{\mu=1}^{P}\vx^{\mu} \vx^{\mu^\top} = \mI$. This assumption can be achieved easily by various data preprocessing methods. For example, it is held exactly for whitened input data. Given the assumption, the derivative is further simplified to: 
\begin{equation*}
    \frac{\partial \loss}{\partial \mW} = \mW - \Sigma^{31},
\end{equation*}

\subsubsection{Faster convergence}
When $\mW$ is initialized as zero matrix, this derivative becomes:$\frac{\partial \loss}{\partial \mW}|_{\mW=0} = - \Sigma^{31}$. Because $\mW$ is updated via gradient descent, during training, the zero-initialized $\mW$ is represented as: $\mW = c \Sigma^{31}$, where $c$ is a scalar scale factor. 

Because the optimal solution of the gradient descent algorithm is achieved when $\mW^{\star} = \Sigma^{31}$, this suggests that: when weights are initialized as zero, the update direction is already aligned with the optimal solution at the beginning of the training. This indicates a faster convergence speed for zero initialization because non-zero initialization requires to adjust both direction and scale during training.

\subsubsection{Better generalization}
As suggested by \cite{ZhangBHRV16}, when weights are initialized at zero, SGD often converges to a solution with minimum norm. \textbf{(will be filled)}

\subsection{Consider multiple layers: deep linear residual model}
We expand our model from a simple linear model to deep linear residual model that consists of multiple linear transformations: $\funcF(\vx,\mW) = (\mW_{L} + \mI) ... (\mW_{1} + \mI) \vx$, where $\mW_L$ ... $\mW_1$ are L matrices, and $\mI$ is the identity matrix. 

\subsubsection{Fixed dimensionality across layers (global minimizer closes to zero)}
In this section, we want to show: for deep linear residual model, the global minimizer is closer to zero as depth becomes larger. This result motivates us to initialize all weights at zero in order to approach to the global minimizer as close as possible. The analysis follows the result from \cite{identity_matters}.

For the simplicity of the analysis, here we assume input $\vx$ and output $\vy$ share the same dimensionality $\sR^{d}$, and the problem is learning a learning transformation $\vy=\mR \vx+\xi, \text { where } \xi \in \mathcal{N}\left(0, I_{d}\right)$ is a d-dimensional spherical Gaussian vector. We also assume all matrices have the same dimensionality where $\mW_L, ..., \mW_1 \in \sR^{d} \times \sR^{d}$.
\begin{restatable}{theorem}{globalminimum}\label{thm:globalminimum}
    (Theorem 2.1 in \cite{identity_matters}) \\
    Suppose $L \geq 3 \gamma$ and $\operatorname{det}(R)>0 .$ Then, there exists a global minimizer $\mW^{\star}$ of the loss $\loss$ with norm
    $$
    \left\|\mW^{\star}\right\| \leq(4 \pi+3 \gamma) / L,
    % \left\|\mW^{\star}\right\| \leq \Theta(1 / L),
    $$
\end{restatable}
where $\gamma:=\max \left\{\left|\log \sigma_{\max }(\mR)\right|,\left|\log \sigma_{\min }(\mR)\right|\right\}$. 

\subsubsection{varying dimensionality across layers (introduce symmetric learning problem)}
Although theorem \ref{thm:globalminimum} motivates us to initialize weights at zero, the fixed dimensionality setting is far from the best practice where high dimensional hidden spaces and non-linearity are equipped to improve the representational power of models. In this section, we will show that when deep linear residual models include higher dimensional hidden spaces, a symmetric learning problem will exist if the weights are initialized at zero or any fixed value.    

Here we consider a simple case first: $\funcF(\vx,\mW) = (\mW^{21} + \mI^{21}) (\mW^{10} + \mI^{10}) \vx$, where $\mW^{21} \in \sR^{N_L \times N_1}$ and $\mW^{10} \in \sR^{N_1 \times N_0}$. We assume $N_1 > N_0,N_L$, suggesting a higher dimensional hidden representation is used. Since the dimensionalities are varied across layers, we need to use dimensionality-varied skip connections $\mI^{10}$ and $\mI^{21}$. We assume two deterministic skip connections follow deterministic expanding or eliminating techniques: 1) $\mI^{10} = (\mI^{00}, 0)^\top \in \sR^{N_1 \times N_0}$ where $\mI^{00} \in \sR^{N_0 \times N_0}$ is an identity matrix, 2) $\mI^{21} = (\mI^{22}, 0) \in \sR^{N_L \times N_1}$ where $\mI^{22} \in \sR^{N_L \times N_L}$ is an identity matrix.

Consider the derivatives wrt. $\mW^{21}$ and $\mW^{10}$:
\begin{equation*}
\begin{aligned}
    \frac{\partial \loss}{\partial \mW^{21}} &= - \sum_{\mu=1}^{P}(\vy^{\mu} \vx^{\mu^\top} - (\mW^{21} + \mI^{21}) (\mW^{10} + \mI^{10}) \vx^{\mu} \vx^{\mu^\top}) (\mW^{10} + \mI^{10})^\top, \\
    \frac{\partial \loss}{\partial \mW^{10}} &= - \sum_{\mu=1}^{P}(\mW^{21} + \mI^{21})^\top (\vy^{\mu} \vx^{\mu^\top} - (\mW^{21} + \mI^{21}) (\mW^{10} + \mI^{10}) \vx^{\mu} \vx^{\mu^\top}). \\
\end{aligned}
\end{equation*}

Since the weights are initialized as zero matrix, we further simplify the derivatives at initialization:
\begin{equation*}
\begin{aligned}
    \frac{\partial \loss}{\partial \mW^{21}}|_{\mW=0} &= - \sum_{\mu=1}^{P}(\vy^{\mu} - \mI^{21} \mI^{10} \vx^{\mu}) (\mI^{10} \vx^{\mu})^\top, \\
    \frac{\partial \loss}{\partial \mW^{10}}|_{\mW=0} &= - \sum_{\mu=1}^{P}\mI^{21^\top} (\vy^{\mu} - \mI^{21} \mI^{10} \vx^{\mu}) \vx^{\mu^\top}. \\
\end{aligned}
\end{equation*}

From a direct matrix calculation, we know that: 1) $(\frac{\partial \loss}{\partial \mW^{21}})_{i,j} = 0$ where $i \in (1,N_L)$ and $j \in (N_L+1, N_2)$, and 2) $(\frac{\partial \loss}{\partial \mW^{10}})_{i,j} = 0$ where $i \in (N_1+1,N_2)$ and $j \in (1, N_1)$. We call the weights that share the same derivative at initialization as \textit{degenerated weights}. The degenerated weights also share the same weight value during training, and thus it strongly limits the power of gradient-based optimization methods. Previous works also name this problem as \textit{symmetric learning problem}. 

In order to break the symmetric, most recent works focus on randomly initializing weights based on Gaussian distribution or Uniform distribution. As mentioned earlier, these random initialization methods inevitably encode biased prior knowledge on weights which might lead to sub-optimal solutions.

To initialize weights at zero while avoiding symmetric learning problem, we propose a new residual network called ZeroResNet. Equipped with orthogonal transformation, we will show that ZeroResNet breaks any symmetric involved during training. 

\subsection{Orthogonality for high-dimensional hidden spaces}
In this section, we will show how orthogonal transformation breaks the symmetric learning problem. Different from the 3-layer network motioned earlier, we apply an orthogonal transformation after each linear mapping: \begin{equation*}
    \funcF(\vx,\mW) = \mQ^{21} (\mW^{21} + \mI^{21}) \mQ^{10} (\mW^{10} + \mI^{10}) \vx
\end{equation*}
where $\mQ^{21} \in \sR^{N_L \times N_L}$ and $\mQ^{10} \in \sR^{N_1 \times N_1}$ are randomly initialized orthogonal matrices, and these orthogonal matrices are fixed through training. The derivatives wrt. $\mW^{21}$ and $\mW^{10}$ at zero are:

\begin{equation*}
\begin{aligned}
    \frac{\partial \loss}{\partial \mW^{21}}|_{\mW=0} &= - \sum_{\mu=1}^{P} \mQ^{21^\top} (\vy^{\mu} - \mI^{21} \mI^{10} \vx^{\mu}) (\mQ^{10} \mI^{10} \vx^{\mu})^\top, \\
    \frac{\partial \loss}{\partial \mW^{10}}|_{\mW=0} &= - \sum_{\mu=1}^{P} \mQ^{10^\top} \mI^{21^\top} \mQ^{21^\top} (\vy^{\mu} - \mI^{21} \mI^{10} \vx^{\mu}) \vx^{\mu^\top}. \\
\end{aligned}
\end{equation*}

Another case is:
\begin{equation*}
    \funcF(\vx,\mW) = (\mW^{21} + \mI^{21}) \mQ^{11^\top} (\mW^{10} + \mQ^{11} \mI^{10}) \vx
\end{equation*}
where $\mQ^{11} \in \sR^{N_1 \times N_1}$ is a randomly initialized orthogonal matrix. This ensures higher-dimensional hidden spaces receive orthogonal transformed inputs and also transform them back to the original space.  The derivatives wrt. $\mW^{21}$ and $\mW^{10}$ at zero are:
\begin{equation*}
\begin{aligned}
    \frac{\partial \loss}{\partial \mW^{21}}|_{\mW=0} &= - \sum_{\mu=1}^{P} (\vy^{\mu} - \mI^{21} \mI^{10} \vx^{\mu}) ( \mI^{10} \vx^{\mu})^\top, \\
    \frac{\partial \loss}{\partial \mW^{10}}|_{\mW=0} &= - \sum_{\mu=1}^{P} \mQ^{11^\top} \mI^{21^\top} (\vy^{\mu} - \mI^{21} \mI^{10} \vx^{\mu}) \vx^{\mu^\top}. \\
\end{aligned}
\end{equation*}




\subsection{Towards zero-initialized deep residual network: ZeroResNet}

\subsubsection{Orthogonal transformation breaks the symmetric}

\subsubsection{Detailed structure description}


==> sections/X-outline.tex <==
\section{Outline}

\begin{enumerate}
    \item Abstract
    \item Introduction
    \item Related Work
    \item Problems of scaled random initialization and symmetric learning
    \item Orthogonality - the symmetric breaker
    \item ZeroResNet - zero initialized residual network
    \item Experiments
    \item Conclusion
\end{enumerate}

==> sections/additional_discussion.tex <==
\section{Additional discussions}

\subsection{Zero-initialized linear model}
\label{sec:zero_linear}

==> sections/old-4-1-method.tex <==
\section{ZerO Initialization for Residual Networks}

In this section, we show how we initialize all the weights to zero for a plain neural network consisting of fully-connected layers. As motivated in the introduction, skip connections allow to mitigate the vanishing gradient problem and possibly avoid it completely. We take the skip connection to the extreme by applying it to every layer in the network, which ensures the input flows to the end even when all layers are blocked. 

In modern neural networks, hidden layers usually need dimensions larger than the input dimension to improve the expressiveness of the network. When a layer has small dimension than the next layer, the conventional identity skip connection does not work as it doesn't match the dimension of the next layer. As we will show it later, common ways to expand the dimension of the skip connection does not work when the weights are initialized to zero. Instead, we propose a special skip connection based on Hadamard transform, which is defined in \ref{eq:hadamard}. 

Overall, we find that the weights can be fully initialized to zero when fully-connected neural networks satisfying:
\begin{itemize}
    \item \emph{\textbf{Every fully-connected layer is associated with a skip connection.}}
    \item \emph{\textbf{Hadamard transform is applied to every skip connection where the dimension needs to be expanded.}}uj
\end{itemize}
We illustrate the above procedures at Figure \ref{fig:methodology}. In next section, we will explain why two design requirements are necessary to train a zero-initialized fully-connected residual network.


==> sections/old-4-desgin.tex <==
\section{Symmetries in deep neural networks}

When backward propagation was first proposed by \citet{<first_backward>}, neural networks were initialized randomly in order to break the symmetry between parameters and hidden features. Although many sophisticated random initialization schemes were designed for deep neural networks, few of studies investigated what are the exact symmetries existed in neural networks when initializing the weights in a deterministic way. In this section, we theoretically identify two levels of symmetries when initializing weights deterministically, and discuss our methodologies used to break the symmetries. 

For simplicity, we limit our focus on a common deterministic initialization scheme that initializes all the weights using a constant value. We denote it as \textit{constant initialization}. We note that zero initialization is a special case of constant initialization, and we will discuss it separately as it requires additional considerations.

We consider a problem of learning a function $\hat{\vy} = \funcF(\vx)$ with parameters $\mW$ by minimizing the squared error $\loss = \frac{1}{2} \norm{\vy - \hat{\vy}}_2^2$. $(\vx,\vy)$ is a sample data and the learning is accomplished via gradient descent. 

\subsection{Level-1 symmetries}

With constant initialization, we first recap a well-known symmetric level existed in standard fully-connected neural networks. We use a simple single layer linear network as a motivation, where $\funcF(\vx) = \mW^2 \, \vh^1$ where $\vh^1 = \mW^1 \, \vx$.  We ignore bias terms and assume input, output and the hidden space with the same dimension of three, as illustrated at Figure \ref{fig:linear_model}. 

The derivative with respect to $\mW^2$ is: $\grad{\loss}{\mW^2} = (y - \hat{y}) \, \vh^{1^{\top}} = (y - \hat{y}) \, (\mW^{1} \, \vx)^{\top}$. Because $\mW^2,\mW^1$ are initialized as a constant value, each entry of $\vh^1 = \mW^{1} \, \vx$ shares the same value, and thus columns of $\grad{\loss}{\mW^2}$ are the same. Therefore, after the first weight updates, the columns of $\mW^2$ share the equivalence. Similarly, because entries of $\grad{\loss}{\vh^1}$ are the same, rows of $\mW^1$ also share the same value after the first weight updates. To be noted, the entry-level equivalences of $\vh^1$ and $\grad{\loss}{\vh^1}$ are preserved even after the first weight updates, and thus we have the following equivalences \textit{during the entire training}:
\begin{equation*}
    \begin{split}
        \mW^{1}_{i,:} &= \mW^{1}_{j,:} \qquad \text{for any } i,j \in 0,1,2 \\
        \mW^{2}_{:,i} &= \mW^{2}_{:,j} \qquad \text{for any } i,j \in 0,1,2
    \end{split}
\end{equation*}
where $\mW^{1}_{i,:}$ and $\mW^{2}_{:,j}$ denote rows and columns of $\mW^{1},\mW^{2}$, respectively. As seen in the example, constant initialization causes the symmetries between parameters and neurons. The symmetries in parameters cause the symmetries in neurons where all neurons in a same layer generate the same output no matter what the input is, such as $\vh^1$ in the example above. This damages the expressiveness of the network because a hidden space has the same representation ability as a single neuron in the space no matter how large the hidden dimension is.

We also generalize this problem from a single layer network to a more general setting. Assume $\funcF(\vx)$ is a deep linear network with $L-1$ layers: $\funcF(\vx) = \mW^L \, \mW^{L-1} \, ... \, \mW^2 \, \mW^1 \, \vx$. Dimension and other settings follow the previous example. We have the following theorem: 
\begin{restatable}[Level-1 symmetries]{theorem}{symmetric}
    \label{thm:symmetric}
    If all the weights $\mW$ in $\funcF(\vx)=\mW^L \, \mW^{L-1} \, ... \, \mW^2 \, \mW^1 \, \vx$ are initialized as a constant $c$, during training, the weights satisfy:
    \begin{equation*}
        \begin{split}
        \mW^{1}_{i,:} &= \mW^{1}_{j,:} \qquad \text{for any } i,j \in 0,...,N-1, \\
        \mW^{l}_{i,p} &= \mW^{l}_{j,q} \qquad \text{for any } l \in 2,...,L-1 \text{  and } i,j,p,q \in 0,...,N-1, \\
        \mW^{L}_{:,p} &= \mW^{L}_{:,q} \qquad \text{for any } p,q \in 0,...,N-1,
        \end{split}
    \end{equation*}
    where $\mW^{l}_{i,:}$ and $\mW^{l}_{:,j}$ are rows and columns of each matrix, respectively. We denote these symmetries as level-1 symmetries.
\end{restatable}
Theorem \ref{thm:symmetric} indicates that rows of the first matrix $\mW^{1}$, columns of the last matrix $\mW^{L}$, and elements of the intermediate matrices $\mW^{l}$ are identical. This result indicates that some symmetries persist in the network under a constant initialization, and thus it degenerates the expressiveness of the network. Moreover, considering a zero initialization, this surely brings the network to the dead neuron problem as the derivatives with respect to all the weights are zero: $\grad{\loss}{\mW^l} = 0 \text{ for } l \in 1,...,L$.

\subsection{Sample diversity and residual connections break level-1 symmetries}

Theorem \ref{thm:symmetric} also shows that there is no equivalence between columns of $\mW^{1}$ or between rows of $\mW^{L}$. This is because \textit{sample diversity} generates varied inputs $\vx$ and varied derivatives with respect to the outputs $\grad{\loss}{\funcF(\vx)}=(y - \hat{y})$. Take $\mW^L$ as an example. Because $\grad{\loss}{\mW^L} = (\vy - \hat{\vy}) \, (\mW^{L-1} \,...\, \mW^{1} \, \vx)^{\top}$, row equivalence of $\grad{\loss}{\mW^L}$ depends on the vector $(\vy - \hat{\vy})$ and the column equivalence depends on the vector $(\mW^{L-1} \,...\, \mW^{1} \, \vx)$. We know that the column equivalence holds as the matrices are initialized by a constant. However, the row equivalence does not hold as entries of $(\vy - \hat{\vy})$ do not share a same value. This is because $\vy$ is randomly sampled from the distribution and the sample diversity ensures the variety of $\vy$. Similarly, sample diversity breaks the column equivalence of $\mW^{1}$ as well.

Given the derivation above, it is obvious that sample diversity fully breaks the symmetries in a constant initialized linear model as the row and column equivalences are broken by inputs and output derivatives. This explains why linear models can be initialized as zero without performance degradation. It also potentially converges to a solution with minimum L2-norm as discussed in \citep{zhang_understanding_2016}.
% option: potentially has faster convergence speed (discuss in the appendix) \ref{sec:zero_linear}

%%%%%
% introduction to feature diversity
% The cause of the symmetries between parameters is the symmetries between features at initialization. For a neural network, the hidden space at every layer is a collection of features computed from the previous layer. When a network is initialized using a constant, except for the first layer, every layer receives identical features no matter what the inputs are. As studied in \citep{feature_diversity}, identical features are detrimental to the training.
%%%%%

% can try in tensorflow playground: http://playground.tensorflow.org

% option: point out this can generalize to an intermediate layer setting
% showing that matrix is the out-product of input vector and gradients
% learning symmetric of linear regression in a compositional function
% $\funcF(\vx^{\mu},\mW) = (f_m \,...\, f_1 \circ h \circ g_n \,...\, g_1)(\vx)$ where $h(\vx)=\mW \, \vx$ and 
% fail: hard to generalize to such a setting, need to define the condition of both vectors that are composed of gradient matrix.

% option: reason why all identity initialization is not good

%%%%%
% put this paragraph after linear regression (or even after introducing everything)
% We also note that some matrices can be initialized as a constant (including zero) without inducing the symmetric. For example, when initializing the matrix in the last layer $\mW^{L}$ as zero, and initializing other layers randomly, there is no symmetric in $\mW^{L}$ during training. At initialization, $\grad{\loss}{\mW^L}$ depends on both vectors $(y - \hat{y})$ and $(\mW^{L-1} \,...\, \mW^{1} \, \vx)$. 
%%%%%

Considering deep linear network in the previous example, sample diversity still can fully break the symmetric when networks are equipped with residual connections. Based on the previous modelling assumption, we add a residual connection for each layer in the network: $\funcF(\vx) = (\mW^{L} + \mI) ... (\mW^{1} + \mI) \vx$, where $\mI$ is the identity matrix. When initializing all weights using a constant value, every layer receives the signals from inputs of the network $\vx$ and derivatives of the network outputs $\grad{\loss}{\mW_L}$, and thus there is no symmetry in any matrix. Therefore, sample diversity can fully break the symmetries in a constant initialized deep linear residual network.

% option: a comparison figure showing the weight distribution difference

We also note that skip connections not only break the symmetries but also ensure perfect signal propagation when initializing all the weights as zero. This is because skip connections ensure non-zero signals during forward and backward propagation. This also works for deep non-linear residual networks given that derivative of the non-linearity exists at zero. 

%%%%%
% Focus on zero initialization + benefits of zero initialization
% As motivated in the introduction, zero initialization does not require a sophisticated design of the initial weight scales to prevent signals from vanishing or exploding at initialization. In addition, zero initialization plays a more important role on the training of residual networks. 

% to-do Add-ons: 1) form as identity mapping at initialization, which helps remove-batch normalization, 2) achieves initial dynamical isometry and no variance explosion and vanishing, 3)close to the global solution

% option: Also, starting from non-zero value is hard to reach a final Gaussian-like distribution (mean zero).
%%%%%

\subsection{Level-2 symmetries}

% However, considering a practical network with high-dimensional hidden spaces, residual networks need to address additional symmetric under zero initialization.
For the deep residual networks discussed above, the dimensions of all hidden spaces are required to be equal to the input dimension. However, for practical residual networks where hidden dimensions are usually different, a constant initialization might introduce additional symmetries.

Follow the single layer network we discussed before, we add skip connections and expand the dimension of $\vh^1$ from 3 to 5: $\funcF(\vx) = (\mW^{2} + \mI^{2}) (\mW^{1} + \mI^{1}) \vx$, where $\mW^{1} \in \sR^{5 \times 3}$ and $\mW^{2} \in \sR^{3 \times 5}$. Since the dimensions are varied across layers, we need to apply dimension varied skip connections $\mI^{1}$ and $\mI^{2}$. When expanding the dimension, we follow a standard practice by applying a constant padding skip connection that duplicates all three features from the previous layer while padding additional two features using a constant value, such as zero or the average of the features. When reducing the dimension, we simply select the top three features from the previous output. The network and skip connections are illustrated at Figure \ref{fig:linear_model}. 

Although the residual network $\funcF(\vx)$ utilizes the sample diversity to break the symmetries, there still exists symmetries in the network due to the high dimensional hidden space. Specifically, during training, there are equivalences between rows $\mW^{1}_{3,:}$ and $\mW^{1}_{4,:}$, and between columns $\mW^{2}_{:,3}$ and $\mW^{2}_{:,4}$. This is because the additional features generated by the constant padding skip connection are identical and do not depend on the network input, which lead to the symmetries in parts of $\mW^{1}$ and $\mW^{2}$. 

Here we consider a more general setting: $\funcF(\vx)=(\mW^{L} + \mI^{L}) ... (\mW^{1} + \mI^{1}) \vx$, where $\vx \in \sR^{M}$, $\vy \in \sR^{N}$, $\mW^{1}$ and $\mI^{1} \in \sR^{K \times M}$, $\mW^{L}$ and $\mI^{L} \in \sR^{N \times K}$, and $\mW^{l}$ and $\mI^{l} \in \sR^{K \times K}$ for any $l \in 2,...,L-1$. Assume $K > M,N$, suggesting the network has $L-1$ high dimensional hidden layers. For $l \in 2,...,L-1$, $\mI^{l}$ is an identity matrix. $\mI^{1}$ is a constant padding skip connection: $\mI^{1} = (\mI^{00}, \bm{c})^\top$ where $\mI^{00} \in \sR^{M \times M}$ is an identity matrix and $\bm{c}$ is a $\sR^{M \times (K-M)}$ matrix with a constant value $c$. Similarly, $\mI^{L}$ preserves the first $N$ features: $\mI^{L} = (\mI^{LL}, \bm{c})$ where $\mI^{LL} \in \sR^{N \times N}$ is an identity matrix and $\bm{c}$ is a ${K \times (K-N)}$ matrix with a constant value $c$.Given all we need, we prove the level-2 symmetries in the following theorem:
\begin{restatable}[Level-2 symmetries]{theorem}{symmetricadditional}\label{thm:symmetricadditional}
    If all the weights $\mW$ in $\funcF(\vx)$ are initialized as a constant, during training, the weights satisfy:
    \begin{equation*}
        \begin{split}
        \mW^{1}_{i,:} &= \mW^{1}_{j,:} \qquad \text{for any } i,j \in M,...,K-1, \\
        \mW^{l}_{i,:} &= \mW^{l}_{j,:} \qquad \text{for any } i,j \in M,...,K-1, \\
        \mW^{l}_{:,p} &= \mW^{l}_{:,q} \qquad \text{for any } p,q \in N,...,K-1, \\
        \mW^{L}_{:,p} &= \mW^{L}_{:,q} \qquad \text{for any } p,q \in N,...,K-1
        \end{split}
    \end{equation*}
\end{restatable}
Theorem \ref{thm:symmetricadditional} indicates that level-2 symmetries happen when the networks have high dimensional hidden spaces with constant padding skip connections. We note that many popular convolutional networks have these design properties as they have large channel dimensions and zero padding skip connections, and thus level-2 symmetries are widely existed. 

% put in the structure section
% For popular convolutional residual networks, their computational logic usually follows expansions of channel dimension and reductions of spatial dimension. For example, ResNet-18 proposed by \citep{resnet} expands the channel dimension from 3 to 512 while reducing thehe first weight updates, the columns of spatial dimension to 1 for each channel in the end. When applying residual connections to channel expanding layers, a standard non-parametric method is duplicating all channels from the previous layer while padding additional channels as zero, which is also called constant padding residual connection.

\subsection{Feature orthogonal transformation breaks level-2 symmetries}

In order to break level-2 symmetries, we propose to apply orthogonal transformation to every dimension expanding skip connection. Given the previous modelling assumption, the network becomes: $\funcF(\vx)=(\mW^{L} + \mI^{L}) ... (\mW^{1} + \mQ \, \mI^{1}) \vx$ where $\mQ$ is a $K \times K$ orthogonal matrix. By using orthogonal matrix $Q$, the features generated by the residual branch $\mQ \, \mI^{1}$ become non-identical and thus break the level-2 symmetries in Theorem \ref{thm:symmetricadditional}.

However, we note that for linear networks, some linear weight correlations still exist even after applying orthogonal transformations. For example, assuming weights are initialized as zero, $\grad{\loss}{\mW^{2}}$ becomes $\mI^{L^{\top}} \, (\vy - \hat{\vy}) \, (\mQ \, \mI^{1} \, x)^{\top}$. \textbf{discuss, to be continued}

% couldn't solve the problem under linear setting + state low-rank issue.

% NEED TO THINK non-linearity breaks the symmetric by using orthogonal transformation (when even receiving identical features) 

% Option: sample diversity is enough to break this symmetric 

% difference from orthogonal initialization: 1) ortho init applies on weights, sometimes need to encode certain scale, 2) ortho init needs to be applied on every weight matrices, but ... 3)ortho init is hard for conv weights but ortho transform on features is easier.

% additional randomness is necessary but it does not need to be applied on weight initialization

% Illustrations: aligned information vs. orthogonal transformed information through non-linearity (think a better way to explain)

\subsection{Zero Initialization}

\subsection{Measuring the symmetries}
To verify the existence of levels of symmetries and the effectiveness of our symmetric breakers, we empirically measure the weight correlations to represent the degree of symmetries during the training. Similar to \citep{identical_feature}, for each weight matrix, we measure the correlations between row vectors and column vectors, respectively. This also measures the row and column equivalences discussed in previous theorems. Given a $M \times N$ weight matrix $\mW$, we define forward correlations $C_f$ and backward correlations $C_b$ as follows:
\begin{equation*}
    \begin{split}
        C_f = \frac{1}{M(M-1)} \sum_{i}^{M} \sum_{i \neq j}^{M} \frac{\mW_{i,:} \cdot \mW_{j,:}}{\norm{\mW_{i,:}}_2 \, \norm{\mW_{i,:}}_2}, \\
        C_b = \frac{1}{N(N-1)} \sum_{i}^{N} \sum_{i \neq j}^{N} \frac{\mW_{:,i} \cdot \mW_{:,j}}{\norm{\mW_{:,i}}_2 \, \norm{\mW_{:,j}}_2}
    \end{split}
\end{equation*}
where $A \cdot B$ denotes a dot product of vectors. \textbf{to be added (depends on the page limit)}

% Measurements: Evolution of weight correlations

%Previous methods to break the symmetric: random weight initialization, dropout or GPU arithmetics

% Compare those methods based on the measurements


==> sections/proofs.tex <==
\section{Proofs for Theorem \ref{thm:symmetric}}

% Placeholder for some theory (wait to see the length)
% Here we consider a more general setting: $\funcF(\vx)=(\mW^{L} + \mI^{L}) ... (\mW^{1} + \mI^{1}) \vx$, where $\vx \in \sR^{M}$, $\vy \in \sR^{N}$, $\mW^{1}$ and $\mI^{1} \in \sR^{K \times M}$, $\mW^{L}$ and $\mI^{L} \in \sR^{N \times K}$, and $\mW^{l}$ and $\mI^{l} \in \sR^{K \times K}$ for any $l \in 2,...,L-1$. Assume $K > M,N$, suggesting the network has $L-1$ high dimensional hidden layers. For $l \in 2,...,L-1$, $\mI^{l}$ is an identity matrix. $\mI^{1}$ is a constant padding skip connection: $\mI^{1} = (\mI^{00}, \bm{c})^\top$ where $\mI^{00} \in \sR^{M \times M}$ is an identity matrix and $\bm{c}$ is a $\sR^{M \times (K-M)}$ matrix with a constant value $c$. Similarly, $\mI^{L}$ preserves the first $N$ features: $\mI^{L} = (\mI^{LL}, \bm{c})$ where $\mI^{LL} \in \sR^{N \times N}$ is an identity matrix and $\bm{c}$ is a ${K \times (K-N)}$ matrix with a constant value $c$. Given all we need, we have the following observation about the symmetries:
% \begin{restatable}[Symmetries]{observation}{symmetricadditional}\label{thm:symmetricadditional}
%     If all the weights $\mW$ in $\funcF(\vx)$ are initialized as a constant, during training, the weights satisfy:
%     \begin{equation*}
%         \begin{split}
%         \mW^{1}_{i,:} &= \mW^{1}_{j,:} \qquad \text{for any } i,j \in M,...,K-1, \\
%         \mW^{l}_{i,:} &= \mW^{l}_{j,:} \qquad \text{for any } i,j \in M,...,K-1, \\
%         \mW^{l}_{:,p} &= \mW^{l}_{:,q} \qquad \text{for any } p,q \in N,...,K-1, \\
%         \mW^{L}_{:,p} &= \mW^{L}_{:,q} \qquad \text{for any } p,q \in N,...,K-1
%         \end{split}
%     \end{equation*}
% \end{restatable}
% Theorem \ref{thm:symmetricadditional} indicates that the symmetries happen when the networks have high dimensional hidden spaces with constant padding skip connections. We note that many popular convolutional networks have these design properties as they have large channel dimensions and zero padding skip connections, and thus the symmetries are widely existed. 

\symmetric*
%to-do
The derivatives with respect to every weight matrices are:
\begin{equation*}
    \begin{split}
        \grad{\loss}{\mW^1} &= (\mW^L \,...\, \mW^2)^{\top} \, (y - \hat{y}) \, \vx^{\top}, \\
        %to-do think about whether we should exclude l=2 and l=L-1 as well
        \grad{\loss}{\mW^l} &= (\mW^L \,...\, \mW^{l+1})^{\top} \, (y - \hat{y}) \, (\mW^{l-1} \,...\, \mW^{1} \, \vx)^{\top} \qquad \text{for } l \in 2,...,L-1, \\
        \grad{\loss}{\mW^L} &= (y - \hat{y}) \, (\mW^{L-1} \,...\, \mW^{1} \, \vx)^{\top}.
    \end{split}
\end{equation*}

\section{Proofs for Theorem \ref{thm:symmetricadditional}}
%Need to modify
\symmetricadditional*
Consider the derivatives wrt. $\mW^{2}$ and $\mW^{1}$:
\begin{equation*}
\begin{aligned}
    \frac{\partial \loss}{\partial \mW^{2}} &= - \sum_{\mu=1}^{P}(\vy^{\mu} \vx^{\mu^\top} - (\mW^{2} + \mI^{2}) (\mW^{1} + \mI^{1}) \vx^{\mu} \vx^{\mu^\top}) (\mW^{1} + \mI^{1})^\top, \\
    \frac{\partial \loss}{\partial \mW^{1}} &= - \sum_{\mu=1}^{P}(\mW^{2} + \mI^{2})^\top (\vy^{\mu} \vx^{\mu^\top} - (\mW^{2} + \mI^{2}) (\mW^{1} + \mI^{1}) \vx^{\mu} \vx^{\mu^\top}). \\
\end{aligned}
\end{equation*}

Since the weights are initialized as zero matrix, we further simplify the derivatives at initialization:
\begin{equation*}
\begin{aligned}
    \frac{\partial \loss}{\partial \mW^{2}}|_{\mW=0} &= - \sum_{\mu=1}^{P}(\vy^{\mu} - \mI^{2} \mI^{1} \vx^{\mu}) (\mI^{1} \vx^{\mu})^\top, \\
    \frac{\partial \loss}{\partial \mW^{1}}|_{\mW=0} &= - \sum_{\mu=1}^{P}\mI^{21^\top} (\vy^{\mu} - \mI^{2} \mI^{1} \vx^{\mu}) \vx^{\mu^\top}. \\
\end{aligned}
\end{equation*}

From a direct matrix calculation, we know that: 1) $(\frac{\partial \loss}{\partial \mW^{2}})_{i,j} = 0$ where $i \in (1,c)$ and $j \in (c+1, b)$, and 2) $(\frac{\partial \loss}{\partial \mW^{1}})_{i,j} = 0$ where $i \in (a+1,b)$ and $j \in (1, b)$. We call the weights that share the same derivative at initialization as \textit{degenerated weights}. The degenerated weights also share the same weight value during training, and thus it strongly limits the power of gradient-based optimization methods. Previous works also name this problem as \textit{symmetric learning problem}. 

==> sections/to-do-sentences.tex <==
A note that skip connection is not necessary, there are other ways to propagate the input information at initialization.

Note that ZerO not only contains weight initialization but also modifies the model structure to ensure a well-conditioned identity initialization. 

A well-conditioned identity initialization: at initialization, each layer receives a Hadamard-transformed input data, such that (a mathematical condition). \textbf{We need a bold concluded statement after the theorems}. Could be: each layer receives a Hadamard-transformed input data, such that (a mathematical condition).

About the efficiency of Hadamard transform: because it is a fixed linear transformation, it can be merged into the nearby operations during the inference. 

Figures: put a big illustration in the beginning, and put the current Figure 1 later.

A further thought: we don't even need a fixed Hadamard transform, but we just need to make sure that the first dimension-increasing matrix contains the transformation.

Empirical thoughts: 
1. For a bottleneck block (with information decreasing than increasing), an additional skip connection is more efficient. 

==> tables/non_bn_benchmark.tex <==
\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lccc}
\toprule
\textbf{Method}               & \textbf{Batch Normalization}         & \textbf{Large Learning Rate}          & \textbf{Test Error} \small{(mean $\pm$ std)} \\
\midrule
Kaiming Init            & \cmark & \cmark &        $23.46 \pm 0.07$            \\
Kaiming Init + Mixup           & \cmark & \cmark &        $23.16 \pm 0.09$           \\
\hline
\small{\textit{(Mixup enabled)}} &&& \\
\textbf{ZerO Init}    & \xmark & \cmark &        $24.52 \pm 0.06$            \\
Fixup Init  & \xmark & \cmark &        $23.85 \pm 0.10$            \\
Kaiming Init & \xmark & \xmark &        $29.91 \pm 0.12$            \\
Xavier Init & \xmark & \cmark &        $25.89 \pm 0.11$            \\
\bottomrule
\end{tabular}
\caption{Benchmarking ResNet-50 without batch normalization on ImageNet}
\label{tab:non_bn_results}
\end{table}
